Power and Energy-efficiency Roofline Model for GPUs

Energy consumption has been a great deal of concern in recent years and developers need to take energy-efficiency into account when they design algorithms. Their design needs to be energy-efficient and low-power while it tries to achieve attainable performance provided by underlying hardware. However, different optimization techniques have different effects on power and energy-efficiency and a visual model would assist in the selection process. In this paper, we extended the roofline model and provided a visual representation of optimization strategies for power consumption. Our model is composed of various ceilings regarding each strategy we included in our models. One roofline model for computational performance and one for memory performance is introduced. We assembled our models based on some optimization strategies for two widespread GPUs from NVIDIA: Geforce GTX 970 and Tesla K80.

==> experiments.tex <==
\section{Experimental Results}
Our model can be employed on different platforms. In this section, we validate our model on actual systems.


\subsection{Power-performance Roofline Model for platforms}
We extracted our model in single- and double-precision modes for platforms in Table \ref{TB_platforms} and present them in Fig. \ref{Fig_precision_platform} expressed in logarithmic scale. Power-performance models for Intel's Core i7 6800K are shown in Fig. \ref{Fig_precision_platform}(a) and (c) for single- and double-precision modes, respectively. A maximally attainable performance for this processor in single-precision mode is 446.4 GFLOP per second with respect to a maximally available power level of 140 Watts.  By disabling FMA operations on the processor, the performance drops to 285.1 GFLOP per second.  If we continue and drop support for Single-Instruction Multiple-Data (SIMD) in our code, we can only achieve 147.8 GFLOP per second. By removing the support for TLP and running the kernel on only one core, the performance drops to 24.6 GFLOP per second. In a double-precision mode, as depicted in Fig. \ref{Fig_precision_platform}(c), the serial mode shows close to a 12.3 GFLOP per second performance. When we enabled TLP without the FMA support, the performance reaches 73.7 GFLOP per second. On the next step, we enabled SIMD and FMA operations that enhanced the performance by reaching to 143.1 and 223.8 GFLOP per second. The ridge points for Core i7 happens at 0.31 and 0.63 Joules per GFLOP for single- and double-precision modes, respectively. 

On the NVIDIA's GTX 970 platform, in single-precision mode, we observed an impressive performance of 3,477.5 and 1,930.7 GFLOP per second with or without FMA utilization, respectively. Fig. \ref{Fig_precision_platform}(b) depicts these results. With less than 0.06 Joules per GFLOP, single-precision computations are considered compute-bound on GTX 970 while more than that is considered to be power-bound. In double-precision mode, as shown in Fig. \ref{Fig_precision_platform}(d) when there is no floating-point multiply-add (FMA) operation, Roofline Toolkit module was able to measures 70.2 GFLOP per second. However, when the utilization of FMA operation on CUDA cores is enabled, the performance nearly doubles and reaches 139.2 GFLOP per second. For a double-precision computation, the threshold between compute-bound and power-bound is 1.59 Joules per GFLOP.


\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{fig_precision_platform}
\caption{Power-performance Roofline Model for Intel Core i7-6800K and NVIDIA Geforce GTX 970 in single- and double-precision mode. \(Peak_\pi\) donates the peak performance of the platform. Numbers in parentheses represent measured performance in GFLOP per second.}
\label{Fig_precision_platform}
\end{figure}


We next tested a set of well-known computational kernels in molecular dynamics applications such as Stencil, GEMM (General Matrix Multiplication), and SpMV. These kernels execute a set of computations on known elements of a matrix, two of which are from the Seven Dwarf set identified by Phil Colella \cite{colella2004seven,kaltofen2014seven,williams2009roofline}. Stencil is a multigrid kernel that updates 8 nearby elements in a 2D matrix \cite{datta2008stencil}. GEMM computes multiplication of two matrices. SpMV kernel computes multiplication of a sparse matrix and a dense vector, followed by saving the result into a vector \cite{williams2009optimization}. 

We chose the Stencil and SpMV benchmarks  from Scalable HeterOgeneous Computing (SHOC) Benchmark Suite \cite{danalis2010scalable}. This suite provides known scientific kernels in several programming models such as CUDA and OpenCL. Besides the abovementioned benchmarks, we executed a simple CUDA matrix multiplication kernel as our GEMM benchmark. For each kernel, we used three data sets for benchmarking in Table \ref{TB_data_sizes}. We studied the outcome of a Stencil kernel by using a 2D square Matrix with a varying number of rows from 1024 to 4096 and studied the outcome from a SpMV kernel by varying the number of rows in the matrix from 8192 to 16384 and studied the outcome from a GEMM kernel by employing different sizes of data shown in Table \ref{TB_data_sizes}. 

We show our measurements from benchmarking in single- and double-precision modes on GPU platforms described in Table \ref{TB_platforms} in the next two subsections. First, we tested them based on a constant data size value while the optimization levels vary. Second, once we choose an optimization level with best performance, we studied the effect of data size on power and energy-efficiency. We showed the data by choosing the median of 100 trial runs with the same configuration.



\subsection{Varying optimization levels under a constant data size}
Figure \ref{fig_fix_data} shows the response of kernels with respect to varying optimization levels. We set the input data size to the highest level (Set 3) and tuned the optimizations on all three kernels by varying precision. For each benchmark there are data points where each data point corresponds to whether FMA operations are exploited by GPU or not.  Our model shows that double-precision computations mostly benefit from FMA operations. For single-precision operations, there is no differences in the outcome on Stencil and SpMV kernels when FMA is enabled.  Noticeably, when FMA was enabled for the GEMM benchmark, it leads to reduction in power consumption from 151 to 134 Watts. Although these three kernels consume almost the same amount of power in a single-precision mode, GEMM benchmark is far more energy-efficient than Stencil and SpMV. It is due to the fact that GEMM is cache-friendly to GPU threads in comparison to Stencil and SpMV. The memory access patterns of the latter kernels suffer from insufficient spatial locality due to being inherently sparse. Table \ref{TB_fixed_data} lists the collected values used in Fig. \ref{fig_fix_data}. 

We observed the same trend on energy-efficiency in a double-precision mode. GEMM is far more energy-efficient than the other two benchmarks for the same reason. While the power consumption increases mildly from 102 to 107 Watts, the energy consumption per each GFLOP decreases from 1.72 to 1.11 Joules per GFLOP. By losing (or trading-off) only 4 Watts (about 4\% of the total power), GEMM significantly improves its energy-efficiency by nearly a factor of two. We also observe that upon enabling FMA optimizations, GEMM kernel leans towards being compute-intensive from power-intensive by approaching the performance roofline. We notice a similar trend for the stencil kernel that by enabling FMA operations its the energy-efficiency improves at the expense of losing a small wage of power.



\subsection{Varying data size at a fixed optimization level}
We  investigated the effect of data size on the performance at a fixed optimization level by running benchmarks in single- or double-precision mode. Results for NVIDIA Geforce GTX 970 platform is shown in Fig. \ref{fig_fix_config}. For these experiments, we enabled FMA operations with -O3 flag on the NVCC compiler and varied the data sets in Table \ref{TB_data_sizes}. We showed that by increasing data size increases, kernels consume more power while their energy efficiency remains the same in most cases. However, single-precision SpMV computations tend to lose energy-efficiency when the data size increases. 

On the other hand, GEMM kernel shows a compute-bound behavior in double-precision mode by remaining close to the peak performance roofline although its single-precision version is power-bound. By increasing the data size, it requires an additional energy under a similar operation protocol on the processor. Hence, the energy-efficiency appears to be relatively insensitive to an increase of data size. For instance, energy-efficiency of double-precision operations for stencil benchmark of Set 1, 2, and 3 are 48, 54, and 55 mJ/GFLOP, respectively. Table \ref{TB_fixed_opt} presents list of collected values used in this section.


\begin{figure}[!t]
\centering
\includegraphics[width=2in]{fix-config}
\caption{Fixed optimization level with different data size. Please refer to Table \ref{TB_data_sizes} for more information on data sizes. Numbers in parentheses represent measured performance in GFLOP per second.}
\label{fig_fix_config}
\end{figure}




==> setup.tex <==
\section{Experimental Setup}
In this section, we discuss our experimental setup and methodologies that we used for benchmarking and measurements.


\subsection{Hardware Setup}
Table \ref{TB_platforms} shows our experimental setup. We tested our model on two separate GPUs with different architectures: NVIDIA Tesla K80 with Kepler architecture, and an NVIDIA Geforce GTX 970 with second generation Maxwell architecture. 


On NVIDIA side, we enabled persistence mode\footnotemark  and set the GPU clock and memory clock to maximum available values recommended by the device;  1,531 MHz and 3,505 MHz, respectively. To do so, we used \textit{nvidia-smi} tool provided by NVIDIA. 

\footnotetext{By enabling persistence mode on NVIDIA platforms, any settings provided by user for core and memory clocks remains persistence between program runs for the driver. We used this feature to set the clock frequency of core and memory of on the GTX 970. It can be enabled using \textit{nvidia-smi} tool with \textit{-pm 1} options.}

To compile our code on Intel processor, \textit{gcc} compiler was used with -O3 by default. Then, we added related flags for SIMD operations and FMA operations. For NVIDIA, we used CUDA programming model and its designated compiler, \textit{nvcc}. Similar approach was used for nvcc too. By exploiting \textit{-fma} flag, we can toggle the usage of FMA operation on NVIDIA's processors. We also investigate the usage of \textit{-use\_fast\_math} flag to boost floating-point operations through optimizations on a set of computation and rounding operations. Besides enabling these optimizations, it will also enable FMA operations by default. Based on our observations, we did not see any improvements from exploiting this flag in comparison to enable only FMA in our experiments. Therefore, we only used results focused on utilization of FMA operations. We also set the data alignment to our favor. On GPU side, we used 32-bit data alignment addresses for variables, while on CPU side, we used 64-bit alignment. 

Maximum attainable power level \(P_{peak}\) for NVIDIA architecture could be collected through \textit{nvidia-smi} tool. Using \textit{-q} flag, the tool reports the maximum power limit of the core, which for GTX 970 we get 222 Watts. On Intel, peak power could be extracted through RAPL interface and also system specifications provided by chip manufacturer company. For the processor in this paper, Core i7 6800K, peak power is reported as 140 Watts. 


\begin{table}[!tb]
% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{Platform specification}
\label{TB_platforms}
\centering
% Some packages, such as MDW tools, offer better commands for making tables
% than the plain LaTeX2e tabular which is used here.

\begin{tabular}{llllll}
\textbf{Platform}& \textbf{Model}   & \textbf{Freq.}  & \textbf{Cores} & \textbf{Ppeak}   & \textbf{Compiler} \\
                 &                  & \textbf{(GHz)}  &                & \textbf{(Watts)} & \\
\hline
\hline
CPU & Intel    & 3.4 & 6                             & 140 & gcc \\ 
    & Core i7  &     & GP\footnotemark               &     & \\
    & 6800K    &     & Cores                         &     & \\
\hline
GPU & NVIDIA   & 1.5  & 1664       & 222 & nvcc \\
    & Geforce  &      & CUDA       &     &  \\
    & GTX 970  &      & Cores      &     & \\
\hline

\end{tabular}

\end{table}

\footnotetext{General Purpose}



\subsection{Benchmarking}
We used Roofline Toolkit package \cite{lo2014roofline} for our investigation. We executed the toolkit program with various configurations to measure the computational ceilings for each platform in our model. It pushes the hardware by reaching its maximum attainable performance under extreme benchmarking conditions. Besides computing performance, reported as GFLOP per second, the attainable memory bandwidth for main memory and L1 cache is measured too. We used this package for collecting our performance measurement data by measuring the above features empirically. 

Thermal Design Power (TDP) is defined as the maximum amount of heat generated by a processor under normal load. It provides system designers a perspective on how to design their cooling system.  However, TDP could not be used as the peak power level because often times the peak power consumption is considered 1.5 times of TDP \cite{hennessy2012computer}. Although we could consider this value to present peak power, it would not be applicable for all platforms; therefore, we used the method mentioned previously, i.e. \textit{nvidia-smi} to find the max power for NVIDIA GPUs and RAPL for Intel processors. 

To measure power and energy of a kernel, no external power meters were used. Instead, we relied on the software Application Programming Interfaces (APIs) provided by the manufacturers. Today, chip manufacturer companies, like Intel and NVIDIA, willingly expose the power consumption to the end-user through a set of APIs. Developers gain insights into energy/power consumption by querying the current power level of their chips (CPU or GPU) conveniently. 


\subsection{Measurement Methodology}
Power was measured through executing a \textit{separate process} on the host. This process measures power consumption of a host or device and record them in its database. The power level of GPU was queried through NVIDIA's library, NVML \cite{nvidiasmi}, in milliwatts unit. For the CPU part, we used Intel's RAPL \cite{rotem2012power, hackenberg2015energy} to measure power consumption. The \textit{separate process} runs in background of the host and queries the power level every few milliseconds. 

To evaluate our method and identify the location of any kernel on our model, we developed Phoenix\footnotemark, a tool consists of a couple of function calls, that tries to measure execution time and energy consumption of any kernel we are focusing on. Figure \ref{Fig_phoenix} shows a diagram of  Phoenix. The following steps demonstrate how it collects data from any region:

\footnotetext{Since our tool is put to sleep and resurrected back to life each time a kernel is met, we chose the name Phoenix for it. --- Wikipedia says: ``In Greek mythology, a phoenix is a long-lived bird that is cyclically regenerated or reborn. Associated with the Sun, a phoenix obtains new life by arising from the ashes of its predecessor.'' --- Available on Github: \textit{\url{https://github.com/milladgit/phoenix}}}

\begin{enumerate}
  \item Upon the start of the program, Phoenix is initialized. In this step, Phoenix creates a thread with an infinite loop on the host. This loop samples power levels for every X milliseconds (X varies by the amount of requested work). Each sample is appended to the end of a buffer inside Phoenix. Each time the buffer is filled up, all the recorded power levels are transferred back to a file on the disk. 
  \item Before entering the kernel, \textit{phoenix\_region\_start} is called. Simply put, it sets the flag (as a static variable shared among threads) that allows the \textit{sampler thread} to start its job. 
  \item The sampler thread starts sampling the power level in parallel with the rest of the application. It wakes up every few milliseconds and samples the power level, and then it goes back into the sleep mode again. 
  \item After the kernel is done, \textit{phoenix\_region\_stop} will announce the end of kernel to the sampler thread by unsetting the shared variable. This will lead the thread to go into polling state until encountering a new kernel. 
  \item At the end of the program, if the buffer is not empty, the rest of the recorded samples are transferred to the file on the disk; then the sampler thread is killed.
\end{enumerate}


\begin{figure}[!t]
\centering
\includegraphics[width=2.25in]{fig_phoenix}
\caption{Phoenix in address space of an application.}
\label{Fig_phoenix}
\end{figure}


After these steps, we calculate energy offline. A definite integral of all recorded power levels over time is computed. This method allows us to precisely evaluate energy value in comparison to using only the power level at the start and at the end of a process (and multiplying it with execution time).


The final note regarding our measurement methodology is about the resolution of the sampling method. Choosing a sampling rate is not straightforward. In general, if the chosen sampling rate is more than what the underlying hardware supports, that could lead to overrated sampling, which does not offer any new information because the same value is repeated multiple times while the hardware is busy for no reason. However, if the chosen sampling rate is less than what the underlying hardware supports, it is likely that information be lost. Considering these conditions, for our experiments, we need to choose an appropriate sampling rate to sample power consumption levels. To that end, we chose 2 milliseconds such that we do not lose useful information. 

%underrated sampling looses information between two consecutive sampling. Consider these conditions, in our experiments, we set the waiting time intervals to 2 milliseconds. 

%thread goes to sleep x ms, things running on gpu, every 2 ms, thread comes up and nvml - what is the power level of GPU, gets the power level, goes to sleep, but for the CPU, computational kernel + phoenxix kernel on the CPU, if this is set to 2ms, it causes the CPU to have more context switches, instead of doing useful work, increasing to 10 ms, for cpu = power value is updated every 10 ms, for the GPU

